Efficient Transfer Learning in Diffusion Models via Adversarial Noise

Diffusion Probabilistic Models (DPMs) have demonstrated substantial promise in image generation tasks but heavily rely on the availability of large amounts of training data. Previous works, like GANs, have tackled the limited data problem by transferring pre-trained models learned with sufficient data. However, those methods are hard to be utilized in DPMs since the distinct differences between DPM-based and GAN-based methods, showing in the unique iterative denoising process integral and the need for many timesteps with no-targeted noise in DPMs. In this paper, we propose a novel DPMs-based transfer learning method, TAN, to address the limited data problem. It includes two strategies: similarity-guided training, which boosts transfer with a classifier, and adversarial noise selection which adaptive chooses targeted noise based on the input image. Extensive experiments in the context of few-shot image generation tasks demonstrate that our method is not only efficient but also excels in terms of image quality and diversity when compared to existing GAN-based and DDPM-based methods.

==> img/rebuttal-ablation.tex <==
\begin{figure}[!t]
    \vskip 0.2in
    \centering
    \includegraphics[width=0.99\textwidth]{img/source/rebuttal-ablation.pdf}
    % \vskip -0.05in
    \caption{This illustrate the DDPM-TAN generated image on FFHQ $\to$ Landscape for with 1, 5, 10 target images. The red border target iamge is for the 1-shot image generation and the red and green border target iamge is for the 5-shot image generation }
    % \vskip -0.2in
\end{figure}

==> img/rebuttal-cls-guieded.tex <==
\begin{figure}[!t]
    \vskip 0.2in
    \centering
    \includegraphics[width=0.99\textwidth]{img/source/cls-guided.pdf}
    % \vskip -0.05in
    \caption{This is the generated image from pre-trained model on Churches only depenied on churches\&landscapes classifier guidance.}
    % \vskip -0.2in
\end{figure}

==> img/rebuttal-display.tex <==
\begin{figure}[!th]
    \vskip 0.2in
    \centering
    \includegraphics[width=0.99\textwidth]{img/source/rebuttal-display.pdf}
    % \vskip -0.05in
    \caption{This is the generated image by DDPM-TAN (Ours) in FFHQ $\rightarrow$ Amedeo's paintings, FFHQ $\rightarrow$ Sketches and Church $\rightarrow$ Haunted houses.}
    % \vskip -0.2in
\end{figure}

==> img/rebuttal-dreambooth.tex <==
\begin{figure}[!th]
    \vskip 0.2in
    \centering
    \includegraphics[width=0.99\textwidth]{img/source/dreambooth.pdf}
    % \vskip -0.05in
    \caption{This is the generated image by dreambooth.}
    % \vskip -0.2in
\end{figure}
